Learning Human Optical Flow

The optical flow of humans is well known to be useful for the analysis of human action. Given this, we devise an optical flow algorithm specifically for human motion and show that it is superior to generic flow methods. Designing a method by hand is impractical, so we develop a new training database of image sequences with ground truth optical flow. For this we use a 3D model of the human body and motion capture data to synthesize realistic flow fields. We then train a convolutional neural network to estimate human flow fields from pairs of images. Since many applications in human motion analysis depend on speed, and we anticipate mobile applications, we base our method on SpyNet with several modifications. We demonstrate that our trained network is more accurate than a wide range of top methods on held-out test data and that it generalizes well to real image sequences. When combined with a person detector/tracker, the approach provides a full solution to the problem of 2D human flow estimation. Both the code and the dataset are available for research.

==> 6analysis.tex <==
\paragraph{Timing Evaluation}
Although some of the methods do quite well on our benchmark, they tend to be slow due to their complex nature. As such, they are not likely to be used in real time applications such as analyzing pedestrians, motion controlled gaming, robotic interactions etc. We show that learning with a good human data can make our model a lot simpler while simultaneously making it faster and accurate for capturing human motion. Our model take 31 ms to estimate optical flow. As such it can run in real time at 32 frames per second.

\paragraph{Network Size}
Employing spatial pyramid structures \cite{ranjan2016optical} to neural network architectures leads to significant reduction of size. As such our network is quite small and can be stored on 7.8 MB of disk space. Our network has a total of 4.2 million learnable parameters making it fast and easy to train.
